Cardinality Estimation in DBMS: A Comprehensive Benchmark Evaluation

Cardinality estimation (CardEst) plays a significant role in generating high-quality query plans for a query optimizer in DBMS. In the last decade, an increasing number of advanced CardEst methods (especially ML-based) have been proposed with outstanding estimation accuracy and inference latency. However, there exists no study that systematically evaluates the quality of these methods and answer the fundamental problem: to what extent can these methods improve the performance of query optimizer in real-world settings, which is the ultimate goal of a CardEst method. In this paper, we comprehensively and systematically compare the effectiveness of CardEst methods in a real DBMS. We establish a new benchmark for CardEst, which contains a new complex real-world dataset STATS and a diverse query workload STATS-CEB. We integrate multiple most representative CardEst methods into an open-source database system PostgreSQL, and comprehensively evaluate their true effectiveness in improving query plan quality, and other important aspects affecting their applicability, ranging from inference latency, model size, and training time, to update efficiency and accuracy. We obtain a number of key findings for the CardEst methods, under different data and query settings. Furthermore, we find that the widely used estimation accuracy metric(Q-Error) cannot distinguish the importance of different sub-plan queries during query optimization and thus cannot truly reflect the query plan quality generated by CardEst methods. Therefore, we propose a new metric P-Error to evaluate the performance of CardEst methods, which overcomes the limitation of Q-Error and is able to reflect the overall end-to-end performance of CardEst methods. We have made all of the benchmark data and evaluation code publicly available at https://github.com/Nathaniel-Han/End-to-End-CardEst-Benchmark.

==> VLDB173-Arxiv/benchmark.tex <==

% !TeX spellcheck = en_US

\section{Our New Benchmark}
\label{sec: bench}

In this section, we design a new benchmark with complex real-world data and diverse multi-table join query workload for evaluating \CE algorithms. To simulate practical scenarios, the benchmark should attain the following properties: 


\indent \underline{\textit{1) Large scale}} with enough tables,  attributes, and  tuples in the full outer join;

\indent \underline{\textit{2) Complex distribution}} with skewed and correlated attributes whose joint distribution can not be modeled in a straightforward manner (e.g. independent assumption);

\indent \underline{\textit{3) Rich join schema}} containing joins of various number of tables and diverse join forms (e.g. star and chain);


\indent \underline{\textit{4) Diverse workload}} with queries covering a wide range of true cardinalities and different number of filtering and join predicates.


To this end, we establish our benchmark on a new real-world dataset with a hand-picked query workload. It overcomes the drawbacks of existing \CE benchmarks and fully fulfills the properties listed above. We describe the details on the data and workload settings in the following content. 

\begin{figure}
	\centering
	\includegraphics[width=6cm]{stats_schema.eps}
	\vspace{-1em}
	\caption{Join relations between tables in STATS.}
	\label{fig: benchjoin}
	\vspace{-1em}
\end{figure}

\myskip
\noindent \underline{\textbf{Data Setting:}}
We adopt the real-world dataset STATS\footnote{\url{https://relational.fit.cvut.cz/dataset/Stats}}
in our benchmark. It is an anonymized dump of user-contributed content on the Stats Stack Exchange network. STATS consumes 658MB storage space with 8 tables and 71 \revise{n./c.} attributes on users, posts, comments, tags, and their relations. A comparison of the statistical information between STATS and IMDB \revise{(the simplified subset supporting JOB-LIGHT)} is shown in Table~\ref{tab: benchmarkstat-data}. We argue that STATS more suitable for \CE benchmark as follows:


\indent \underline{\textit{1) Larger scale:}} 
STATS has more data tables and a larger number of \revise{n./c. attributes} than \revise{the simplified} IMDB. Moreover, its full outer join size is four orders of magnitude larger.

\indent \underline{\textit{2) More complex data distribution:}} 
The distribution skewness of STATS and attribute correlation is more significant than \revise{the simplified} IMDB.
Moreover, STATS has $3 \times$ more attributes with a larger domain size, suggesting its PDF is much harder to model.


\indent \underline{\textit{3) Larger query space:}} 
\revise{
Each table in STATS has $1$ to $8$ n./c. attributes to be filtered while the simplified IMDB contains at most two in each table. 
}
Moreover, STATS's full outer join size is much larger than \revise{the simplified} IMDB.
These two aspects provide STATS a larger query space varying in cardinality and predicate numbers.

\indent \underline{\textit{4) Richer join settings:}} 
The join relations between all tables in STATS are shown in Figure~\ref{fig: benchjoin}.
\revise{The simplified} IMDB contains only star joins between primary key and foreign keys (i.e. 5 join relations). Whereas, STATS has richer and more diverse join types varying in the number of joined tables (from $2$ to $8$), join forms (chain, star, and mixture of these two), and join keys (PK-FK and FK-FK).



\begin{table}[t]
	\caption{Comparison of IMDB \revise{(simplified subset to fit JOB-LIGHT workload)} and STATS dataset.}
	\vspace{-1em}
	\scalebox{0.87}{
		\begin{tabular}{c|c|cc}
			\hline
			\rowcolor{mygrey}
			\textbf{Criteria} & \textbf{Item} & \textbf{IMDB} & \textbf{STATS} \\ \hline
			\multirow{4}{*}{Scale} &\# of tables & 6 & 8 \\
			&\# of \revise{n./c.} attributes & 8 & 23 \\
			&\# of \revise{n./c.} attributes per table & 1--2 & 1--8 \\
			&full outer join size & $2\cdot 10^{12}$ & $3\cdot10^{16}$ \\ \hline
			\multirow{3}{*}{Data}& total attribute domain size & 369, 563 & 578, 341 \\
			&average distribution skewness & 9.159 & 21.798 \\
			&average pairwise correlation & 0.149 & 0.221 \\ \hline
			\multirow{2}{*}{Schema} & join forms & star & star/chain/mixed\\
			& \# of join relations & 5 & 12\\ \hline
		\end{tabular}
		\label{tab: benchmarkstat-data}
	}
	\vspace{-2em}
\end{table}


\myskip
\noindent \underline{\textbf{Query Workload Setting:}}
We generate and then carefully handpick a query workload STATS-CEB on STATS to fulfill both practicality and diversity. The generation process is done in two phases. 


In the first phase, we generate $70$ representative join templates based on the join schema in Figure~\ref{fig: benchjoin}, each of which specifies a distinct join pattern covering a set of tables. For these join templates, we do not consider: 
1) cyclic joins as most of the ML-based \CE algorithms~\cite{yang2020neurocard, hilprecht2019deepdb, zhu2020flat, wu2020bayescard} do not support them;
and 2) non-equal joins as they rarely occur in practice and many \CE algorithms process them in the same way as many-to-many joins.
We manually check and retain each join template if it has occurred in the log data of StackExchange%\footnote{\url{https://stackexchange.com}} 
or has its real-world semantics.
To reduce redundancy, we also ensure that these join templates are not very similar (e.g. only differ in inner or outer join conditions).

In the second phrase after deriving these $70$ join templates, we generate $146$ queries with $1-4$ queries for each template as the testing query workload STATS-CEB. We make sure all the generated filter predicates reflect real-world semantics and diversify in multiple perspectives.
In comparison to JOB-LIGHT (illustrated in Table~\ref{tab: benchmarkstat-workload}), we find the following advantages of STATS-CEB:


\indent  \underline{\textit{1) More diverse queries:}} 
STATS-CEB contains twice queries as JOB-LIGHT with $3 \times$ more join templates covering a wider range of the number of joined tables.

\indent \underline{\textit{2) Richer join types:}}
Unlike JOB-LIGHT benchmark with only star joins, STATS-CEB contains queries with chain joins and complex mixed join forms. Moreover, JOB-LIGHT only contains queries with one-to-many PK-FK joins, whereas STATS-CEB includes queries with many-to-many FK-FK joins.

\indent \underline{\textit{3) More filter predicates:}}
STATS-CEB contains queries with up to 16 distinct filter predicates, which is $4 \times$ larger than JOB-LIGHT.

\indent \underline{\textit{4) Wider range of true cardinality:}} 
The cardinality range of STATS-CEB is an order of magnitude larger than JOB-LIGHT. The largest query in STATS-CEB has true cardinality of 20 billion, which is $3 \times$ larger than that of the JOB-LIGHT benchmark.


\myskip
\noindent \underline{\textbf{Summary:}}
\revise{
Our new benchmark with STATS dataset and STATS-CEB query workload are very comprehensive  with more complex data, more skewed distribution, more diverse queries and more complicated join settings. According to our evaluation results in the following Sections~5--7, this new \CE benchmark helps to find more insights over existing \CE algorithms that have not been discovered in previous works.
}


\begin{table}[t]
	\caption{Comparison of JOB-LIGHT and STATS-CEB benchmark query workload.}
	\vspace{-1em}
	\scalebox{0.9}{
		\begin{tabular}{c|cc}
			\hline
			\rowcolor{mygrey}
			\textbf{Item} & \textbf{JOB-LIGHT} & \textbf{STATS-CEB} \\ \hline
			\# of queries & 70 & 146 \\
			\# of joined tables & 2--5 & 2--8 \\
			\# of join templates & 23 & 70 \\
			\# of filtering \revise{n./c.} predicates & 1--4 & 1--16 \\
			join type & PK-FK & PK-FK/FK-FK\\
			true cardinality range & 9 --- $9\cdot10^9$ & 200 --- $2\cdot10^{10}$  \\ \hline
		\end{tabular}
	}
	\label{tab: benchmarkstat-workload}
	\vspace{-1em}
\end{table}

==> VLDB173-Arxiv/dynamic.tex <==
% \section{Dynamic Performance Analysis}
\section{What Other Aspects of \CE Methods Matter?}
\label{sec: dynamic}

In addition to \CE's improvement in execution time, we discuss model practicality aspects in this section: inference latency (in Section~\ref{sect6.1}), model size and training time (in Section~\ref{sect6.2}), and model update speed and accuracy (in Section~\ref{sect6.3}). 
\revise{We only compare the recently proposed \CE methods, which have been proved to significantly improve the \textsf{PostgreSQL} baseline, namely \textsf{PessEst}, \textsf{MSCN}, \textsf{NeuroCard}$^E$, \textsf{BayesCard}, \textsf{DeepDB}, and \textsf{FLAT}.}

\revise{
\begin{table}
  %\vspace{-0.5em}
	\caption{\revise{OLTP/OLAP Performance on STATS-CEB.}}
	\vspace{-1.2em}
	\label{tab:TPAP}
	%\begin{tiny}
	\scalebox{0.71}{
		\begin{tabular}{ccc|cc}
			\hline
			\rowcolor{mygrey}
			\revise{\bf Methods} & \revise{\bf \textsf{TP Exec. Time}} & \revise{\bf \textsf{TP Plan Time}} & \revise{\bf \textsf{AP Exec. Time}} & \revise{\bf \textsf{AP Plan Time}} \\ \hline
			 \textsf{PostgreSQL}& 44.7s & 4.8s (9.7\%) & 11.32h & 20.3s ($0.05\%$)   \\ 
			 \textsf{TrueCard} & 8.2s & 4.8s (36.9\%) & 5.68h & 20.3s ($0.1\%$) \\ 
			 \textsf{PessEst} & 19.3s & 8.4s (30.3\%) & 6.09h & 35.4s ($0.16\%$) \\ 
			 \textsf{MSCN} & 15.7s & 8.2s (34.3\%) & 8.11h & 38.0s ($0.13\%$) \\ 
			 \textsf{NeuroCard$^E$} & 26.3s & 73s (73.5\%) & 11.84h & 350s ($0.81\%$) \\ 
			 \textsf{BayesCard} & 10.7s & 7.3s (40.6\%) & 7.15h & 27.4s ($0.11\%$) \\ 
			 \textsf{DeepDB}    & 11.5s & 33.6s (74.5\%) & 6.46h & 135s ($0.58\%$) \\ 
			 \textsf{FLAT}  & 14.3s & 41.5s (74.4\%) & 5.80h & 396s ($1.86\%$) \\ \hline
  		\end{tabular}
	}
	%\end{tiny}
	\vspace{-2em}
\end{table}}

\subsection{Inference Latency}
\label{sect6.1}

The end-to-end query time is comprised of query execution and planning time, the latter of which is determined by the \CE method's inference latency. Commercial DBMS normally has a negligible planning time due to their simplified cardinality estimator and engineering effort to accelerate the inference speed. However, the inference latency of some ML-based data-driven methods can approach one second per sub-plan query, which slows down the end-to-end query execution time. 
\revise{To further illustrate the importance of inference latency, we divide the STATS-CEB queries into OLTP and OLAP two workloads based on the query execution time. We report the results in Table~\ref{tab:TPAP} and derive the following observation.} 



\smallskip
\noindent \revise{\textbf{O7: Inference latency can have a significant impact on the OLTP workload but a trivial impact on the OLAP workload.}
On OLTP workload of STATS-CEB, we observe that the planning time composes a large proportion of total end-to-end time. Specifically, some ML-based methods' (\textsf{NeuroCard}$^E$, DeepDB, and FLAT) inference speeds are relatively slow. Although their execution time on OLTP workload is faster than \textsf{PostgreSQL}, they have worse end-to-end performance because of the long planning time. 
For OLAP workload of STATS-CEB, the \CE methods' planning time is much shorter than their execution time because OLAP workload contains extremely long-run queries. In this case, the quality of the generated query plans overshadows the slow inference latency.
Therefore, we believe that \CE methods targeting different workloads should fulfill different objectives. For OLTP workload, a desirable method should have fast inference speed, whereas the methods targeting OLAP workload can have high inference latency as long as they can produce high-quality query plans.} 


%Specifically, revisiting Table~\ref{tab:overall}, we observe that the pure execution time for \revise{\textsf{NeuroCard}$^E$} on the JOB-LIGHT benchmark is near-optimal but the overall runtime is significantly longer than \textsf{FLAT} and \textsf{BayesCard} because of its slow inference procedure on CPU. Admittedly, for some extremely long-run queries (e.g. query 57 of STATS-CEB), inference latency is overshadowed by the execution time. However, for most queries, inference latency does have a large impact on the overall end-to-end query time because planning one query will request the \CE methods to estimate dozens of its sub-plan queries. Therefore, we claim that a \CE method is not very practical if it takes more than couple hundreds milliseconds to estimate one sub-plan query.

%Alternatively, the effect of slow model inference latency is less severe for extremely long-run queries. For example, query 57 of STATS-CEB described in Section~\ref{sec: static} runs for more than one hour. A planning time 

Figure~\ref{fig: practicality} reports the average inference latencies of all sub-queries in the workload for each method. 
Their inference speed can be ranked as \textsf{BayesCard} $>$ \revise{\textsf{NeuroCard}$^E$(GPU)} $>$ \textsf{FLAT}/\textsf{DeepDB} $>>$ \revise{\textsf{NeuroCard}$^E$}. 
The newly proposed inference algorithms on BN provide \textsf{BayesCard} with a very fast and stable inference speed on both benchmarks. 
However, the inference speeds of \textsf{FLAT} and \textsf{DeepDB} are not as stable because they tend to build much larger models with more computation circuits for the more complicated database STATS.
The inference process of \textsf{NeuroCard} requires a large number of progressive samples and its underlying DNN is computationally demanding on CPUs. Therefore, we observe that the inference speed is greatly improved by running it on GPUs. 

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{practicality_new.eps}
	\vspace{-2.5em}
	\caption{\revise{Practicality aspects of \CE algorithms.}}
	\vspace{-2.5em}
	\label{fig: practicality}
\end{figure}

\subsection{Model Deployment}
\label{sect6.2}
\revise{Figure~\ref{fig: practicality} reports the model size and training time of all aforementioned methods. We do not report \textsf{PessEst} because it is a model-free method that does not need training. 
Based on the results of STATS-CEB query, we derive the following observation.}

\noindent \textbf{O8: BN-based \CE approach is very friendly for system deployment.}
\revise{First of all, the BN-based approaches, such as \break \textsf{BayesCard}, are generally interpretable and predictable, thus easy to debug for DBMS analytics.}
More importantly, a \CE method friendly for system deployment should have faster training time and lightweight model size and \textsf{BayesCard} has the dominant advantage over the other ML-based data-driven methods in these two aspects because of its underlying Bayesian model.
Specifically, from both training time and model size aspects, these methods can be ranked as \textsf{BayesCard} $<<$ \textsf{FLAT}/\textsf{DeepDB} $<$ \revise{\textsf{NeuroCard}$^E$}. We provide the detailed reasoning as follows.

\textsf{BayesCard} proposes an accelerated model construction process of BN using probabilistic programming. Its model training time is roughly 100 times faster than the other three data-driven methods. Moreover, the BNs in \textsf{BayesCard}, which utilize the attribute conditional independence to reduce the model redundancy, are naturally compact and lightweight.

\textsf{FLAT} and \textsf{DeepDB} recursively learn the underlying FSPN and SPN models. 
Their training time is less stable and varies greatly with the number of highly correlated attributes in the datasets. 
Thus, we observe a much longer training time on STATS than on the IMDB dataset for these two methods.
The SPNs in \textsf{DeepDB} iteratively split the datasets into small regions, aiming to find local independence between attributes within each region. 
However, in presence of highly correlated attributes (e.g. STATS), the SPNs tend to generate a long chain of dataset splitting operation, leading to long training time and a very large model size. The FSPNs in \textsf{FLAT} effectively address this drawback of SPNs by introducing the factorize operation but their training time and model size suffer greatly for datasets with a large number of attributes (e.g. STATS) because of the recursive factorize operations.

\revise{The training of \textsf{NeuroCard}$^E$ is particularly long and its size is also the largest on STATS because its join schema does not form a tree. As mentioned in Section~\ref{sec: plan-algo}, the original \textsf{NeuroCard} only supports tree-structured schemas. 
Thus, \textsf{NeuroCard}$^E$ extracts $16$ tree sub-structures from STATS schema graph and train one model for each tree. Therefore, we argue that extending \textsf{NeuroCard} for non-tree-structured schemas can greatly improve its practicality.}



\subsection{Model Update}
\label{sect6.3}
Model update is a crucial aspect when deploying a \CE method in OLTP databases. Frequent data updates in these DBs require the underlying \CE method to swiftly update itself and adjust to the new data accurately. In the following, we first provide our observation regarding the updatability of ML-based query-driven methods and then provide the update experimental settings and results for ML-based data-driven methods on the STATS dataset.

\smallskip
\noindent \textbf{O9: Existing query-driven \CE methods are impractical for dynamic DBs.} The query-driven models require a large amount of executed queries to train their model, which might be unavailable for a new DB and very time-consuming to generate (e.g. 146 STATS-CEB queries take more than ten hours to execute). More importantly, they need to recollect and execute the queries whenever datasets change or query workload shifts. Therefore, they can not keep up with the frequent data update in dynamic DBs.

\smallskip
\noindent \underline{\textbf{Experimental Settings:}} To simulate a practical dynamic environment, we split the STATS data into two parts based on the timestamps of tuples. We first train a stale model for each method on the data created before 2014 (roughly $50\%$) and insert the rest of the data to update these models. We only test the data insertion scenario since some methods (\revise{\textsf{NeuroCard}$^E$} and \textsf{DeepDB}) do not support data deletion. We use the update algorithm in these methods' publicly available source code. 

\begin{table}
	\caption{Update performance of \CE algorithms.}
	\vspace{-1em}
	\label{tab:update}
	%\begin{tiny}
	\scalebox{0.8}{
		\begin{tabular}{@{}ccccc@{}}
			\toprule
			\rowcolor{mygrey}
			\bf Criteria & \bf \revise{\textsf{NeuroCard}$^E$} & \bf \textsf{BayesCard} & \bf \textsf{DeepDB} & \bf \textsf{FLAT} \\ \cmidrule{1-5}
			Update time & 5,569s & \textbf{12s} & 248s  & 360s \\
			Original E2E time (Table~\ref{tab:overall}) &11.85h &7.16h &6.46h &5.80h \\
			E2E time after update & 13.94h & 7.16h & 6.72h & 7.04h \\ \cmidrule{1-5}
		\end{tabular}
	}
	%\end{tiny}
	\vspace{-2em}
\end{table}

\noindent \underline{\textbf{Experimental Results:}} 
As shown in Table~\ref{tab:update}, we record the time these methods take to update their stale models and evaluate the end-to-end query performance of the updated models on STATS-CEB queries. We also cite the original model performance from Table~\ref{tab:overall} as comparison baselines. We first summarize the most important observation based on this table and then provide detailed reasoning from the update speed and accuracy perspectives.

\smallskip
\noindent \textbf{O10: Data-driven \CE methods have the potential to keep up with fast data update and can be applied in dynamic DBs.} Specifically, \textsf{BayesCard} takes $12s$ to update itself for an insertion of millions of tuples on multiple tables in the DB. More important, its end-to-end performance is unaffected by this massive update, thus very suitable for dynamic DBs.  

\textbf{Update speed} of these methods can be ranked as \textsf{BayesCard} $>>$ \textsf{DeepDB} $>$ \textsf{FLAT} $>$ \revise{\textsf{NeuroCard}$^E$}. \textsf{BayesCard} preserves its underlying BN's structure and only incrementally updates the model parameters. Since its model size is relatively small, the update speed is more than $20$ times faster than others. \textsf{DeepDB} and \textsf{FLAT} also preserves their underlying structure of SPN and FSPN but as their structures are significantly larger, the incrementally updating their model parameters still take a large amount of time. 


\textbf{Update accuracy} can be ranked as \textsf{BayesCard} $>$ \textsf{DeepDB} $>$ \textsf{FLAT} $>$ \revise{\textsf{NeuroCard}$^E$}. \textsf{BayesCard}'s underlying BN's structure captures the inherent causality, which is unlikely to change when data changes. Therefore, \textsf{BayesCard} can preserve its original accuracy after model update (i.e. same as its comparison baseline). The structures of SPN in \textsf{DeepDB} and FSPN in \textsf{FLAT} are learned to fit the data before the update and cannot extrapolate well to the newly inserted data. Therefore, only updating the model parameters will cause modeling inaccuracy (i.e. we observe a drop in their end-to-end performance when compared with their baselines).







==> VLDB173-Arxiv/prelim.tex <==

\section{Preliminaries and Background}
\label{sec: prelim}

In this section, we introduce some preliminaries and background, including a formal definition of the cardinality estimation (\CE) problem,
a brief review on representative \CE algorithms and a short analysis on existing \CE benchmarks.

\myskip
\noindent \underline{\textbf{\CE Problem:}}
In the literature, \CE is usually defined as a statistical problem. Let $T$ be a table with $k$ attributes $A = \{A_1, A_2, \dots, A_k \}$. $T$ could either represent a single relational table or a joined table.
In this paper, we assume each attribute $A_i$ for each $1 \leq i \leq k$ to be either categorical (whose values can be mapped to integers) or continuous, whose domain (all unique values) is denoted as $D_i$. 
Thereafter, any selection query $Q$ on $T$ can be represented in a canonical form: $Q = \{A_1 \in R_1 \wedge A_2 \in R_2 \wedge \cdots \wedge A_n \in R_n\}$, where $R_i \subseteq D_i$ is the constraint region specified by $Q$ over attribute $A_i$ (i.e. filter predicates). Without loss of generality, we have $R_i = D_i$ if $Q$ has no constraint on $A_i$. Let $\Card(T, Q)$ denote the \emph{cardinality}, i.e., the exact number of records in $T$ satisfying all constraints in $Q$. The \CE problem requires estimating $\Card(T, Q)$ as accurately as possible without executing $Q$ on $T$. 

\revise{
In this paper, we concentrate on evaluating these selection queries on numerical/categorical (n./c.) attributes. We do not consider `LIKE'' (or pattern matching) queries on string attributes due to two reasons: 
1) commercial \CE methods for ``LIKE''  queries in DBMS often use magic numbers~\cite{psql2020, sqlserver2019, mysql2020, mdb2020}, which are not meaningful to evaluate;
and 2) \CE solutions for n./c. queries mainly consider how to build statistical models summarizing attribute and/or query distribution information. Whereas, \CE methods for ``LIKE'' queries ~\cite{sun2019end, shetiya2020astrid, mikolov2013distributed} focus on applying NLP techniques to summarize semantic information in strings. Thus, they tackle with different technical challenges and statistical \CE methods can not effectively support ``LIKE'' queries.
}

\myskip
\noindent \underline{\textbf{\CE Algorithms:}}
There exist many \CE methods in the literature, which can be classified into three classes as follows:

\emph{Traditional \CE methods}, such as histogram~\cite{selinger1979access} and sampling~\cite{leis2017cardinality,heimel2015self,kiefer2017estimating}, are widely applied in DBMS and generally based on simplified assumptions and expert-designed heuristics. 
\revise{
Many variants are proposed later to enhance their performance.
Histogram-based variants include multi-dimensional histogram based methods~\cite{poosala1997selectivity, deshpande2001independence, gunopulos2000approximating, gunopulos2005selectivity, muralikrishna1988equi, wang2003multi}, correcting and self-tuning histograms with query feedbacks~\cite{bruno2001stholes, srivastava2006isomer, khachatryan2015improving, fuchs2007compressed} and updating statistical summaries in DBMS~\cite{stillger2001leo, wu2018towards}.
Sampling-based variants include query-driven kernel-based methods~\cite{heimel2015self,kiefer2017estimating}, index based  methods~\cite{leis2017cardinality} and random walk based  methods~\cite{zhao2018random, li2016wander}.
Some other work, such as the sketch based method~\cite{cai2019pessimistic}, explores a new direction for \CEend.
}

\textit{ML-based query-driven \CE methods} try to learn a model to map each featurized query $Q$ to its cardinality $\Card(T, Q)$ directly. Some ML-enhanced methods improve the performance of \CE methods by using more complex models such as DNNs~\cite{kipf2018learned} or gradient boosted trees~\cite{dutt2019selectivity}.

\textit{ML-based data-driven \CE methods} are independent of the queries. They regard each tuple in $T$ as a point sampled according to the joint distribution $P_T(A) = P_T(A_1, A_2, \dots, A_n)$. 
Let $P_T(Q) = P_T(A_1 \in R_1, A_2 \in R_2, \cdots , A_n \in R_n)$ be the probability specified by the region of $Q$. Then, we have $\Card(T, Q) = P_T(Q) \cdot |T|$ so \CE problem could be reduced to model the probability density function (PDF) $P_T(A)$ of table $T$. 
A variety of ML-based models have been used in existing work to represent $P_T(A)$, the most representative of which includes deep auto-regression model~\cite{yang2019deep,yang2020neurocard,hasan2019multi} and probabilistic graphical models (PGMs) such as
Bayesian networks (BN)~\cite{tzoumas2011lightweight, getoor2001selectivity, wu2020bayescard}, SPN~\cite{hilprecht2019deepdb}, and FSPN~\cite{zhu2020flat}. 
\revise{
In addition, some methods proposed recently such as~\cite{wu2021unified} try to integrate both query and data information for \CEend.
}

\myskip
\noindent \underline{\textbf{\CE Benchmark:}}
Literature works have proposed some benchmark datasets and query workloads for \CE evaluation. We analyze their pros and cons as follows:

1) The synthetic benchmarks such as TPC-C~\cite{leis2015good}, TPC-H~\cite{tpch2021} and TPC-DS~\cite{tpcds2021} and Star Schema benchmarks (SSB)~\cite{o2009star} contain real-world data schemas and synthetic generated tuples. They are mainly used for evaluating query engines but not suitable for \CE because their data generator makes oversimplified assumptions on the joint PDF of attributes, such as uniform distribution and independence. 
However, real-world datasets are often highly skewed and correlated~\cite{leis2015good}, which are more difficult for \CE. 

2) IMDB dataset with its JOB workload~\cite{leis2015good} is a well-recognized benchmark, containing complex data and string ``LIKE'' queries. 
\revise{
To evaluate statistical \CE methods on n./c. queries only, most of the existing works~\cite{kipf2018learned,yang2019deep,yang2020neurocard,hilprecht2019deepdb,zhu2020flat} use the JOB-LIGHT query workload containing 70 selection queries with varied number of joining tables. However, these queries touch only 8 n./c. attributes within six tables of IMDB and the joins between these tables are only star joins centered at one table. 
Thus, this simplified IMDB dataset and its workload cannot comprehensively evaluate the performance of nowadays \CE algorithms on more complex data and varied join settings.} On the other hand, some works~\cite{yang2020neurocard, negi2021flow} generate queries on the IMDB dataset including ``LIKE'' queries which are not supported by most of recent statistical methods.

Apart from these well-established and general-purpose benchmarks, there also exist other benchmarks with specific purposes. For example, Wang~\cite{wang2020ready} presents a series of real-world datasets to analyze whether existing \CE algorithms are suitable to be deployed into real-world DBMS. However, it is only conducted on single-table datasets, which can not reflect the behavior of these models in more practical multi-table settings. 

\myskip
\noindent \underline{\textbf{Summary:}}
A surge of \CE algorithms built on top of statistical models has been proposed in the literature, especially in the last decade. However, existing \CE benchmarks are not sufficient to comprehensively evaluate their performance.



==> VLDB173-Arxiv/workflow.tex <==

% !TeX spellcheck = en_US

\section{Evaluation Plan}
\label{sec: plan}


We aim to evaluate how \CE algorithms behave in a real DBMS, including the end-to-end improvement on optimizing query plans and other practicality aspects, on our new benchmark. 
This section introduces the detailed evaluation plan. Section~\ref{sec: plan-algo} presents all baseline \CE algorithms chosen to be evaluated, Section~\ref{sec: plan-sys} describes our implementation method and system settings, and Section~\ref{sec: plan-met} lists the evaluation metrics of our interests.
 
 \subsection{\CE Algorithms}
 \label{sec: plan-algo}

\revise{
We identify and choose twelve representative \CE algorithms across the three classes (traditional, ML-based query-driven, and ML-based data-driven) reviewed in Section~\ref{sec: prelim}. The selection principles and details of algorithms in each class are elaborated as follows.
}

%\myskip

\noindent
\revise{
\underline{\textbf{Traditional \CE Algorithms:}}
In this class, we choose five algorithms along the technical directions:
1) for histogram-based methods, we evaluate \textsf{PostgreSQL} and \textsf{MultiHist}, which applies the one-dimensional and multi-dimensional histograms for \CEend;
2) for sampling-based methods, we evaluate the uniformly random sampling \textsf{UniSample} method and the more advanced \textsf{WJSample} method for join sampling;
and 3) for other methods, we evaluate \textsf{PessEst}, a recent proposed method that exhibit state-of-the-art performance in some aspects. 
The details are as follows:
}

%\indent 1) \textsf{\underline{{\revise{SimpleHist}}}}~\cite{selinger1979access} assumes all attributes are mutually independent and maintains a 1-D (cumulative) histogram to represent $P_{T}(A_i)$ for each attribute $A_i$. The probability $P_T(Q)$ can then be easily obtained by multiplying all $P_{T}(R_i)$ together. It has been widely applied in DBMS such as SQL Server~\cite{sqlserver2019}. For continuous attributes, we set its binning size to 100.

\indent
\revise{1) \textsf{\underline{{PostgreSQL}}}~\cite{psql2020} refers to the histogram-based \CE method used in the well-known DBMS PostgreSQL. It assumes that all attributes are mutually independent and maintains a 1-D (cumulative) histogram to represent $P_{T}(A_i)$ for each attribute $A_i$. The probability $P_T(Q)$ can then be easily obtained by multiplying all $P_{T}(R_i)$ together. In addition, optimization strategies such as collecting the most common value and industrial implementation are used to enhance the performance.
}

\indent
\revise{
2) \textsf{\underline{{MultiHist}}}~\cite{poosala1997selectivity} identifies subsets of correlated attributes and model them as multi-dimensional histograms. We use the implementation provided in the repository~\cite{yang2019naru}. We do not compare with the variant methods DBHist~\cite{deshpande2001independence}, GenHist~\cite{gunopulos2000approximating,gunopulos2005selectivity} and 
VIHist~\cite{wang2003multi} over~\cite{poosala1997selectivity} since their improvements are not very significant and their open-sourced implementations are not provided.
}

\indent 3) \textsf{\underline{{\revise{UniSample}}}}~\cite{leis2017cardinality,zhao2018random} makes no assumption but randomly fetches records from $T$ on-the-fly according to $P_{T}(A)$ to estimate the probability $P_{T}(Q)$. It is also widely used in DBMS such as MySQL~\cite{mysql2020} and MariaDB~\cite{mdb2020}. We set the sampling size to $10^4$.

\indent
\revise{
4) \textsf{\underline{{\revise{WJSample}}}}~\cite{li2016wander} designs a random walk based method called wander join to sample tuples from multiple tables. It has been integrated into DBMSs and exhibits favorable performance in a recent study~\cite{park2020gcare}. The method~\cite{zhao2018random} then improves from biased to unbiased sampling. We do not compare with it to avoid redundancy.
}

%\indent
\revise{
5) \textsf{\underline{{\revise{PessEst}}}}~\cite{cai2019pessimistic} leverages 
randomized hashing and data sketching to tighten the bound for multi-join queries. It is a new class of estimator as it never underestimates the cardinality. Meanwhile, it has been verified to perform well in real world DBMS.
}

\revise{
We do not compare with the other variants of traditional methods~\cite{bruno2001stholes, srivastava2006isomer, khachatryan2015improving, fuchs2007compressed, stillger2001leo, wu2018towards, heimel2015self,kiefer2017estimating, leis2017cardinality} as they do not exhibit significantly better performance or provide open-source implementation.}
%As reported in the evaluation results of recent work~\cite{yang2019deep, yang2020neurocard, hilp2019deepdb, hasan2019multi}, they are verified to perform much worse than the ML-based \CE methods.

\myskip

\noindent 
\revise{
\underline{\textbf{ML-Based \CE Algorithms:}}
In our evaluation, we choose four query-driven (\textsf{MSCN}, \textsf{LW-XGB}, \textsf{LW-NN} and \textsf{UAE-Q}) and four data-driven (\textsf{NeuroCard}, \textsf{BayesCard}, \textsf{DeepDB} and \textsf{FLAT}) \CE methods. They are representative as they apply different statistical models, and exhibit state-of-the-art performance using each model. Specifically, for query-driven methods, \textsf{MSCN}, \textsf{LW-XGB}/\textsf{LW-NN} and \textsf{UAE-Q} use deep neural networks, classic lightweight regression models and deep auto-regression models to learn the mapping functions, respectively. For the data-driven methods, they build the data distribution utilizing deep auto-regression models and three probabilistic graphical models: BN, SPN, and FSPN, respectively. They use different techniques to balance estimation accuracy, inference efficiency, and model size. Besides, we also evaluate \textsf{UAE}, an extension of \textsf{UAE-Q} using both query and data information.
The details are as follows:
}

\indent 6) \textsf{\underline{MSCN}}~\cite{kipf2018learned} is a deep learning method built upon the multi-set convolutional network model. The features of attributes in table $T$, join relations in query $Q$, and predicates of query $Q$ are firstly fed into three separate modules, where each is comprised of a two-layer neural network. Then, their outputs are averaged, concatenated, and fed into a final neural network for estimation. 
 
\indent 7) \textsf{\underline{LW-XGB}} and 8) \textsf{\underline{LW-NN}}~\cite{dutt2019selectivity}
 formulate the \CE mapping function as a regression problem and apply gradient boosted trees and neural networks for regression, respectively. Specifically, \textsf{LW-XGB} applies the XGBoost~\cite{chen2016xgboost} as it attains equal or better accuracy and estimation time than both LightGBM~\cite{ke2017lightgbm} and random forests~\cite{svetnik2003random} for a given model size.  As the original models only support single table queries, we extend them to support joins with an additional neural network to combine single-table information.

\indent 
\revise{
9) \textsf{\underline{UAE-Q}}~\cite{wu2021unified} applies the deep auto regression models to learn the mapping function. It proposes differentiable progressive sampling via the Gumbel-Sotfmax trick to enables deep auto-regression models to learn from queries.
}

For above query-driven \CE methods, we automatically generate $10^5$ queries as the training examples to train these models. 

%\myskip

10) \revise{\underline{\textsf{NeuroCard}}~\cite{yang2020neurocard}, the multi-table extension of \textsf{Naru}~\cite{yang2019deep}, is built upon a deep auto-regression model.}
It decomposes the joint PDF $P_{T}(A) = P_{T}(A_1) \cdot \prod_{i=2}^{k}  P_{T}(A_i|  A_1, A_2,  \dots, A_{i - 1})$ according to the chain rule and model each (conditional) PDF parametrically by a 4-layer DNN ($4 \times 128$ neuron units). All \revise{tables} can be learned together using a \revise{single} masked auto-encoder~\cite{made}. Meanwhile, a progressive sampling technique~\cite{liang2020variable} is provided to sample points from the region of query $Q$ to estimate its probability. We set the sampling size to $8, 000$. 
We omit a very similar method in~\cite{hasan2019multi} as it has \revise{slightly worse} performance than \textsf{NeuroCard}. 
\revise{Worth noticing that the original \textsf{NeuroCard} method is only designed for datasets with tree-structured join schema. On our STATS benchmark with cyclic join schema, we partition the schema into multiple tree-structured join schemas and build one \textsf{NeuroCard} model for each schema. To avoid ambiguity, we denote this extension method as \textsf{NeuroCard}$^E$ in the following content.}


%\footnote{We confirm this by email in  correspondence to the authors of~\cite{hasan2019multi}.}.


11) \textsf{\underline{BayesCard}}~\cite{wu2020bayescard} is fundamentally based on BN, which models the dependence relations among all attributes as a directed acyclic graph. Each attribute $A_i$ is assumed to be 
conditionally independent of the remaining ones given its parent attributes $A_{\text{pa}(i)}$ so the joint PDF $\Pr_{T}(A) = \prod_{i = 1}^{k} \Pr_{T}(A_i | A_{\text{pa}(i)})$. 
\textsf{BayesCard} revitalizes \textsf{BN} using probabilistic programming to improve its inference and model construction speed (i.e., learning the dependence graph and the corresponding probability parameters). Moreover, it adopts the advanced ML techniques to process the multi-table join queries, which significantly increases its estimation accuracy over previous BN-based \CE methods~\cite{getoor2001selectivity, tzoumas2011lightweight, dasfaa2019}, which will not be evaluated in this paper. We use the Chow-Liu Tree~\cite{chow1968approximating} based method to build the structure of \textsf{BayesCard} and apply the complied variable elimination algorithm for inference.



\indent 12) \textsf{\underline{DeepDB}}~\cite{hilprecht2019deepdb}, based on sum-product networks (SPN)~\cite{poon2011sum,desana2020sum}, approximates $P_T(A)$ by recursively decomposing it into local and simpler PDFs. Specifically, the tree-structured SPN contains sum node to split $P_T(A)$ to multiple $P_{T'}(A)$ on tuple subset $T' \subseteq T$, product node to decompose $P_{T}(A)$ to $\prod_{S}P_{T}(S)$ for independent set of attributes $S$ and leaf node if $P_{T}(A)$ is a univariate PDF. The SPN structure can be learned by splitting table $T$ in a top-down manner. Meanwhile, the probability of $\Pr_{T}(Q)$ can be obtained in a bottom-up manner with time cost linear in the SPN's node size. 

\indent 13) \textsf{\underline{FLAT}}~\cite{zhu2020flat}, based on factorize-split-sum-product networks (FSPN)~\cite{wu2020fspn}, improves over SPN by
adaptively decomposing $P_T(A)$ according to the attribute dependence level. It adds the factorize node to split $P_T$ as $P_T(W) \cdot P_T(H | W)$ where $H$ and $W$ are highly and weakly correlated attributes in $T$. $P_T(W)$ is modeled in the same way as SPN. $P_T(H | W)$ is decomposed into small PDFs by the split nodes until $H$ is locally independent of $W$. Then, the multi-leaf node is used to model the multivariate PDF $P_T(H)$ directly. Similar to SPN, the FSPN structure and query probability can be recursively obtained in a top-down and bottom-up fashion, respectively. 

For both \textsf{DeepDB} and \textsf{FLAT}, we set the RDC thresholds to $0.3$ and $0.7$ for filtering independent and highly correlated attributes, respectively. Meanwhile, we do not split a node when it contains less than $1\%$ of the input data.

%\myskip

\indent 
\revise{
14) \textsf{\underline{UAE}}~\cite{wu2021unified} extends the \textsf{UAE} method by unifiying both query and data information using the auto-regression model. It is a representative work aiming at closing the gap between data-driven and query-driven \CE methods.
}

\myskip

\noindent 
\underline{\textbf{Remarks:}}
For each \CE algorithm, we adopt the publicly available implementation~\cite{hilp2019deepdb, yang2019naru, yang2020sb} if the authors provide it and otherwise implement it by ourselves. For other hyper-parameters, if they are known to be a trade-off of some metrics, we choose the default values recommended in the original paper. Otherwise, we run a grid search to explore the combination of their values that largely improves the end-to-end performance on a validation set of queries. Notice that, each of our evaluated \CE algorithms is an independent and universal tool that can be easily integrated into common DBMS. There have also been proposed some \CE modules~\cite{sun2019end, wu2021unified} that are optimized together with other components in a query optimizer in an end-to-end manner. We do not compare with them as they do not fit our evaluation framework.



\subsection{Implementation and System Settings}
\label{sec: plan-sys}

To make our evaluation more realistic and convincing, we integrate each \CE algorithm into the query optimizer of PostgreSQL~\cite{psql2020}, a well-recognized open-source DBMS. Then, the quality of each \CE method can be directly reflected by the end-to-end query runtime with their injected cardinality estimation.

Before introducing the details of our integration strategy, we introduce an important concept called \textit{sub-plan query}. For each SQL query $Q$, each \textit{sub-plan query} is a query touching only a subset of tables in $Q$.
%\footnote{In DBMS, sub-query refers to the nested query in the \textsf{where} clause, which is different for the sub-plan query concept.}. 
The set of all these queries is called \textit{sub-plan query space}. For the example query $A \bowtie B \bowtie C$, its sub-plan query space contains queries on $A \bowtie B$, $A \bowtie C$, $B \bowtie C$, $A$, $B$, and $C$ with the corresponding filtering predicates. The built-in planner in DBMS will generate the sub-plan query space, estimate their cardinalities, and determine the optimal execution plan. For example, the sub-plan queries $A$, $B$, and $C$ only touch a single table, their \CE results may affect the selection of table-scan methods, i.e. index-scan or seq-scan. The sub-plan queries $A \bowtie B$, $A \bowtie C$, and $B \bowtie C$ touch two tables. Their cardinalities may affect the join order, i.e. joining $A \bowtie B$ with $C$ or $A \bowtie C$ with $B$, and the join method, i.e. nested-loop-join, merge-join, or hash-join. Therefore, the effects of a \CE method on the final query execution plan are entirely decided by its estimation results over the sub-plan query space.

To this end, in our implementation, 
we overwrite the function ``\textsf{calc\_joinrel\_size\_estimate}'' in the planner of PostgreSQL to derive the sub-plan query space for each query in the workload. 
Specifically, every time the planner needs a cardinality estimation of a sub-plan query, the modified function ``\textsf{calc\_joinrel\_size\_estimate}'' will immediately capture it.
Then, we call each \CE method to estimate the cardinalities of the sub-plan queries and inject the estimations back into PostgreSQL. Afterward, we run the compiler of PostgreSQL on $Q$ to generate the plan. It will directly read the injected cardinalities produced by each method. Finally, we execute the query with the generated plan. In this way, we can support any \CE method without a large modification on the source code of PostgreSQL. We can report the total time (except the sub-plan space generation time) as the end-to-end time cost of running a SQL query using any \CE method.

For the environment, we run all of our experiments in two different Linux Servers. The first one 
with 32 Intel(R) Xeon(R) Platinum 8163 CPUs @ 2.50GHz, one Tesla V100 SXM2 GPU and 64 GB available memory is used for model training. The other one with 64 Intel(R) Xeon(R) E5-2682 CPUs @ 2.50GHz is used for the end-to-end evaluation on PostgreSQL.


 
 \subsection{Evaluation Metrics}
 \label{sec: plan-met}
 
Our evaluation mainly focuses on \emph{quantitative} metrics that directly reflect the performance of \CE algorithms from different aspects. We list them as follows:

\indent 1) \text{\underline{End-to-end time}} of the query workload, including both the query plan generation time and physical plan execution time. It serves as the ``gold-standard'' for \CE algorithm, since improving the end-to-end time is the ultimate goal for optimizing \CE in query optimizers. 
\revise{
We report the end-to-end time of \textsf{TrueCard}, which injects the true cardinalities of all sub-plan queries into PostgreSQL. Ideally if the cost model is very accurate, \textsf{TrueCard} can obtain the optimal plan with shortest time. For a fixed PostgreSQL cost model, we find \textsf{TrueCard} can obtain the optimal query plan for most of the time. Thus, this could serve as a good baseline.
}

\indent 2) \text{\underline{Inference latency}} reflects the time cost for \CE, which directly relates to the query plan generation time. It is crucial as \CE needs to be done numerous times in optimizing the plan of each query. Specifically, an accurate \CE method may be very time-costly in inference. Despite the fast execution time of the plans generated by this method, the end-to-end query performance can be poor because of its long plan generation time.

\indent 3) \text{\underline{Space cost}} refers to the \CE model size. A lightweight model is also desired as it is convenient to transfer and deploy.

\indent 4) \text{\underline{Training cost}} refers to the models' offline training time. 

\indent 5) \text{\underline{Updating speed}} reflects the time cost for \CE models update to fit the data changes. For real-world settings, this metric plays an important role as its underlying data always updates with tuples insertions and deletions.

Besides these metrics, \cite{wang2020ready} proposed some \emph{qualitative metrics} related to the stability, usage, and deployment of \CE algorithms and made a comprehensive analysis. Thus, we do not consider them in this paper.
In the following, we first evaluate the overall end-to-end performance of all methods in Section~\ref{sec: static}. Then, we analyze the other practicality aspects in Section~\ref{sec: dynamic}. At last, we point out the drawbacks of existing evaluation metric and propose a new metric as its potential substitution in Section~\ref{sec:analysis}.
 

